Research and Development for HI Intensity Mapping

Development of the hardware, data analysis, and simulation techniques for large compact radio arrays dedicated to mapping the 21 cm line of neutral hydrogen gas has proven to be more difficult than imagined twenty years ago when such telescopes were first proposed. Despite tremendous technical and methodological advances, there are several outstanding questions on how to optimally calibrate and analyze such data. On the positive side, it has become clear that the outstanding issues are purely technical in nature and can be solved with sufficient development activity. Such activity will enable science across redshifts, from early galaxy evolution in the pre-reionization era to dark energy evolution at low redshift.

==> author_HI_Tech.tex <==
R\'{e}za Ansari$^{1}$,
Evan J. Arena$^{2,3}$,
Kevin Bandura$^{4,5}$,
Adam Beardsley$^{6}$,
Philip Bull$^{7,8}$,
Emanuele Castorina$^{9}$,
Tzu-Ching Chang$^{10,11}$,
Simon Foreman$^{12}$,
Josef Frisch$^{13}$,
Daniel Green$^{14}$,
Dionysios Karagiannis$^{15}$,
Adrian Liu$^{7,8,16}$,
Kiyoshi W. Masui$^{17}$,
P. Daniel Meerburg$^{18,19,20,22,22}$,
Laura B. Newburgh$^{23}$,
Andrej Obuljen$^{24,25,26}$,
Paul O'Connor$^{2}$,
Olivier Perdereau$^{1}$,
Benjamin Saliwanchik$^{23}$,
J. Richard Shaw$^{27}$,
Chris Sheehy$^{2}$,
An\v{z}e Slosar$^{2}$,
Kendrick Smith$^{28}$,
Paul Stankus$^{29}$,
Albert Stebbins$^{30}$,
%Peter Timbie$^{30}$,
Francisco Villaescusa-Navarro$^{31}$,
and Martin White$^{7}$


%%% 

\begin{raggedright}
\setlength{\columnsep}{18pt}
\begin{multicols}{2}

$^{1}$ \ParisSud \\
$^{2}$ \BNL \\
$^{3}$ \StonyBrook \\
$^{4}$ \WVU \\
$^{5}$ \WVUGWAC \\
$^{6}$ \ASU \\
$^{7}$ \UCB \\
$^{8}$ \RAL \\
$^{9}$ \UCBP \\
$^{10}$ \JPL \\
$^{11}$ \Caltech \\
$^{12}$ \CITA \\
$^{13}$ \SLAC \\
$^{14}$ \UCSD \\
$^{15}$ \UNIPD \\
$^{16}$ \McGill \\
$^{17}$ \MIT \\
$^{18}$ \kavli \\
$^{19}$ \ioa \\
$^{20}$ \damtp \\
$^{21}$ \RUG \\
$^{22}$ \VSI \\
$^{23}$ \Yale \\
$^{24}$ \SISSA \\
$^{25}$ \INFN \\
$^{26}$ \UWaterloo \\
$^{27}$ \UBC \\
$^{28}$ \PI \\
$^{29}$ \ORNL \\
$^{30}$ \FNAL \\
%$^{30}$ \UWMadison \\
$^{31}$ \CCA \\


\normalsize
\end{multicols}
\end{raggedright}


==> endorser_HI_Tech.tex <==
Zeeshan Ahmed$^{1}$, 
David Alonso$^{2}$, 
Mustafa A. Amin$^{3}$, 
R\'{e}za Ansari$^{4}$, 
Evan J. Arena$^{5,6}$, 
Kevin Bandura$^{7,8}$, 
Adam Beardsley$^{9}$, 
Philip Bull$^{10,11}$, 
Emanuele Castorina$^{12}$, 
Tzu-Ching Chang$^{13}$, 
Romeel Dav\'e$^{14}$, 
Alexander van Engelen$^{15,9}$, 
Aaron Ewall-Wice$^{13}$, 
Simone Ferraro$^{16}$, 
Simon Foreman$^{15}$, 
Josef Frisch$^{1}$, 
Daniel Green$^{17}$, 
Gilbert Holder$^{18}$, 
Daniel Jacobs$^{9}$, 
Joshua~S.~Dillon$^{19}$, 
Dionysios Karagiannis$^{20,21}$, 
Alexander A. Kaurov$^{22}$, 
Lloyd Knox$^{23}$, 
Emily Kuhn$^{24}$, 
Adrian Liu$^{25}$, 
Yin-Zhe Ma$^{26}$, 
Kiyoshi W. Masui$^{27}$, 
Thomas McClintock$^{5}$, 
Kavilan Moodley$^{26}$, 
Moritz M\{u}nchmeyer$^{28}$, 
Laura B. Newburgh$^{24}$, 
Andrei Nomerotski$^{5}$, 
Paul O'Connor$^{5}$, 
Andrej Obuljen$^{29}$, 
Hamsa Padmanabhan$^{15}$, 
David Parkinson$^{30}$, 
Olivier Perdereau$^{4}$, 
David Rapetti$^{31,32}$, 
Benjamin Saliwanchik$^{24}$, 
Neelima Sehgal$^{33}$, 
J. Richard Shaw$^{34}$, 
Chris Sheehy$^{5}$, 
Erin Sheldon$^{5}$, 
Raphael Shirley$^{35}$, 
Eva Silverstein$^{36}$, 
Tracy Slatyer$^{27,22}$, 
An\v{z}e Slosar$^{5}$, 
Paul Stankus$^{5}$, 
Albert Stebbins$^{37}$, 
Peter T. Timbie$^{38}$, 
Gregory S. Tucker$^{39}$, 
William Tyndall$^{5,24}$, 
Francisco Villaescusa-Navarro$^{40}$, 
Dallas Wulf$^{25}$, 


%%% 

 $^{1}$ \SLAC \\
$^{2}$ \Oxford \\
$^{3}$ \Rice \\
$^{4}$ \ParisSud \\
$^{5}$ \BNL \\
$^{6}$ \drexel \\
$^{7}$ \WVU \\
$^{8}$ \WVUGWAC \\
$^{9}$ \ASU \\
$^{10}$ \QMUL \\
$^{11}$ \UWC \\
$^{12}$ \UCBP \\
$^{13}$ \JPL \\
$^{14}$ \ED \\
$^{15}$ \CITA \\
$^{16}$ \LBL \\
$^{17}$ \UCSD \\
$^{18}$ \UrbanaC \\
$^{19}$ \UCB \\
$^{20}$ \UNIPD \\
$^{21}$ \INFNPD \\
$^{22}$ \IAS \\
$^{23}$ \UCD \\
$^{24}$ \Yale \\
$^{25}$ \McGill \\
$^{26}$ \KwaZuluNatal \\
$^{27}$ \MIT \\
$^{28}$ \PI \\
$^{29}$ \WCA \\
$^{30}$ \KASSI \\
$^{31}$ \CUBoulder \\
$^{32}$ \NPPSFAmes \\
$^{33}$ \StonyBrook \\
$^{34}$ \UBC \\
$^{35}$ \IAC \\
$^{36}$ \Stanford \\
$^{37}$ \FNAL \\
$^{38}$ \UWMadison \\
$^{39}$ \Brown \\
$^{40}$ \CCA \\


